DesCert: Design for Certification

The goal of the DARPA Automated Rapid Certification Of Software (ARCOS) program is to "automate the evaluation of software assurance evidence to enable certifiers to determine rapidly that system risk is acceptable." As part of this program, the DesCert project focuses on the assurance-driven development of new software. The DesCert team consists of SRI International, Honeywell Research, and the University of Washington. We have adopted a formal, tool-based approach to the construction of software artifacts that are supported by rigorous evidence. The DesCert workflow integrates evidence generation into a design process that goes from requirements capture and analysis to the decomposition of the high-level software requirements into architecture properties and software components with assertional contracts, and on to software that can be analyzed both dynamically and statically. The generated evidence is organized by means of an assurance ontology and integrated into the RACK knowledge base.

==> FutureEvidence.tex <==
% Future work evidence description goes here
\section{Future Work on  Evidence Generation}\label{sec:FutureEvidence}

==> conops.tex <==
We have been in regular discussion with TA3 teams (CLARISSA and AACE) to plan how we will iterate over the
assurance case.  First, we as a TA1 team will develop an assurance plan with a draft \emph{Plan for Software Aspects of Certification} (PSAC) document outlining the 
putative assurance argument
along with the high-level claims, arguments, and evidence.  The TA3 team responds with queries for clarification
and explanation on this plan.  The TA3 team then develops a detailed assurance case with defeaters and counter-defeaters.  The TA1 team then delivers the claims and evidence supporting the TA3 assurance argument.  TA3 evaluates
the claims and evidence to see how well they support the assurance argument and ask for additional evidence
in order to patch any weaknesses.  The interaction between TA1 and TA3 takes place through the TA2 Rack-in-a-Box
ontology where the claims and evidence are represented either as data (in JSON form) or metadata (in CSV format).



==> formal_clr_hrl_afs.tex <==








==> toolqual.tex <==
% Tool qualification evidence goes here

We are following the template laid down by the RTCA DO-178C guidance for evidence production.
As part of this, we are also creating tool qualification evidence to demonstrate that the
tools have been validated for use within the assurance case, and that these tools have been
properly integrated into the semantic workflow.  Tool qualification evidence can include
test cases, witnesses, and self-analysis.  We are currently examining tool qualification
evidence for Radler, Checker Framework, Sally, SeaHorn, Clear, and Text2Test.  The DO-330
guidelines for tool qualification are quite onerous, and we are restricting out attention to the
test analysis claims for tool qualification.  The tool qualification evidence also
includes informal semantics definitions for the tools and supporting languages.  


==> tools_usage.tex <==


\textcolor{red}{tbd}
\textcolor{red}{Put Refernce to Earlier Diagram of Evidence Tools  here}

